Seeing your sleep stage: cross-modal distillation from EEG to infrared video

It is inevitably crucial to classify sleep stage for the diagnosis of various diseases. However, existing automated diagnosis methods mostly adopt the "gold-standard" lectroencephalogram (EEG) or other uni-modal sensing signal of the PolySomnoGraphy (PSG) machine in hospital, that are expensive, importable and therefore unsuitable for point-of-care monitoring at home. To enable the sleep stage monitoring at home, in this paper, we analyze the relationship between infrared videos and the EEG signal and propose a new task: to classify the sleep stage using infrared videos by distilling useful knowledge from EEG signals to the visual ones. To establish a solid cross-modal benchmark for this application, we develop a new dataset termed as Seeing your Sleep Stage via Infrared Video and EEG ($S^3VE$). $S^3VE$ is a large-scale dataset including synchronized infrared video and EEG signal for sleep stage classification, including 105 subjects and 154,573 video clips that is more than 1100 hours long. Our contributions are not limited to datasets but also about a novel cross-modal distillation baseline model namely the structure-aware contrastive distillation (SACD) to distill the EEG knowledge to infrared video features. The SACD achieved the state-of-the-art performances on both our $S^3VE$ and the existing cross-modal distillation benchmark. Both the benchmark and the baseline methods will be released to the community. We expect to raise more attentions and promote more developments in the sleep stage classification and more importantly the cross-modal distillation from clinical signal/media to the conventional media.

==> samples/ref.tex <==
\bibitem{ref1}
de Goederen R, Pu S, Viu M S, et al. Radar-based sleep stage classification in children undergoing polysomnography: a pilot-study[J]. Sleep Medicine, 2021, 82: 1-8.
\bibitem{ref2}
Deng B, Xue B, Hong H, et al. Decision tree based sleep stage estimation from nocturnal audio signals[C]//2017 22nd International Conference on Digital Signal Processing (DSP). IEEE, 2017: 1-4.
\bibitem{ref3}
Korkalainen H, Aakko J, Duce B, et al. Deep learning enables sleep staging from photoplethysmogram for patients with suspected sleep apnea[J]. Sleep, 2020, 43(11): zsaa098.
\bibitem{ref4}
Yi R, Enayati M, Keller J M, et al. Non-invasive in-home sleep stage classification using a ballistocardiography bed sensor[C]//2019 IEEE EMBS International Conference on Biomedical & Health Informatics (BHI). IEEE, 2019: 1-4.
\bibitem{ref5}
Quan S F, Howard B V, Iber C, et al. The sleep heart health study: design, rationale, and methods[J]. Sleep, 1997, 20(12): 1077-1085.
\bibitem{ref6}
Zhang G Q, Cui L, Mueller R, et al. The National Sleep Research Resource: towards a sleep data commons[J]. Journal of the American Medical Informatics Association, 2018, 25(10): 1351-1358.
\bibitem{ref7}
Goldberger A L, Amaral L A N, Glass L, et al. PhysioBank, PhysioToolkit, and PhysioNet: components of a new research resource for complex physiologic signals[J]. circulation, 2000, 101(23): e215-e220.
\bibitem{ref8}
O'reilly C, Gosselin N, Carrier J, et al. Montreal Archive of Sleep Studies: an open‐access resource for instrument benchmarking and exploratory research[J]. Journal of sleep research, 2014, 23(6): 628-635.
\bibitem{ref9}
Fraiwan L, Lweesy K, Khasawneh N, et al. Classification of sleep stages using multi-wavelet time frequency entropy and LDA[J]. Methods of information in Medicine, 2010, 49(03): 230-237.
\bibitem{ref10}
Jiang D, Lu Y, Yu M A, et al. Robust sleep stage classification with single-channel EEG signals using multimodal decomposition and HMM-based refinement[J]. Expert Systems with Applications, 2019, 121: 188-203.
\bibitem{ref11}
Liang S F, Kuo C E, Hu Y H, et al. Automatic stage scoring of single-channel sleep EEG by using multiscale entropy and autoregressive models[J]. IEEE Transactions on Instrumentation and Measurement, 2012, 61(6): 1649-1657.
\bibitem{ref12}
Eldele E, Chen Z, Liu C, et al. An attention-based deep learning approach for sleep stage classification with single-channel eeg[J]. IEEE Transactions on Neural Systems and Rehabilitation Engineering, 2021, 29: 809-818.
\bibitem{ref13}
JIA Z, LIN Y, ZHANG H, et al. Sleep stage classification model based ondeep convolutional neural network[J]. Journal of ZheJiang University (Engineering Science), 2020, 54(10): 1899-1905.
\bibitem{ref14}
Cai X, Jia Z, Tang M, et al. Brainsleepnet: Learning multivariate eeg representation for automatic sleep staging[C]//2020 IEEE International Conference on Bioinformatics and Biomedicine (BIBM). IEEE, 2020: 976-979.
\bibitem{ref15}
Jia Z, Lin Y, Wang J, et al. Multi-view spatial-temporal graph convolutional networks with domain generalization for sleep stage classification[J]. IEEE Transactions on Neural Systems and Rehabilitation Engineering, 2021, 29: 1977-1986.
\bibitem{ref16}
Jia Z, Lin Y, Wang J, et al. GraphSleepNet: Adaptive Spatial-Temporal Graph Convolutional Networks for Sleep Stage Classification[C]//IJCAI. 2020: 1324-1330.
\bibitem{ref17}
Phan H, Andreotti F, Cooray N, et al. Joint classification and prediction CNN framework for automatic sleep stage classification[J]. IEEE Transactions on Biomedical Engineering, 2018, 66(5): 1285-1296.

\bibitem{ref18}
Hinton G, Vinyals O, Dean J. Distilling the knowledge in a neural network[J]. arXiv preprint arXiv:1503.02531, 2015, 2(7).
\bibitem{ref19}
Ba J, Caruana R. Do deep nets really need to be deep?[J]. Advances in neural information processing systems, 2014, 27.
\bibitem{ref20}
Buciluǎ C, Caruana R, Niculescu-Mizil A. Model compression[C]//Proceedings of the 12th ACM SIGKDD international conference on Knowledge discovery and data mining. 2006: 535-541.
\bibitem{ref21}
Girdhar R, Tran D, Torresani L, et al. Distinit: Learning video representations without a single labeled video[C]//Proceedings of the IEEE/CVF International Conference on Computer Vision. 2019: 852-861.
\bibitem{ref22}
Komodakis N, Zagoruyko S. Paying more attention to attention: improving the performance of convolutional neural networks via attention transfer[C]//ICLR. 2017.
\bibitem{ref23}
Yim J, Joo D, Bae J, et al. A gift from knowledge distillation: Fast optimization, network minimization and transfer learning[C]//Proceedings of the IEEE conference on computer vision and pattern recognition. 2017: 4133-4141.
\bibitem{ref24}
Park W, Kim D, Lu Y, et al. Relational knowledge distillation[C]//Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition. 2019: 3967-3976.
\bibitem{ref25}
Chen Y, Xian Y, Koepke A, et al. Distilling audio-visual knowledge by compositional contrastive learning[C]//Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition. 2021: 7016-7025.
\bibitem{ref26}
Tung F, Mori G. Similarity-preserving knowledge distillation[C]//Proceedings of the IEEE/CVF International Conference on Computer Vision. 2019: 1365-1374.
\bibitem{ref27}
Liu Y, Chen K, Liu C, et al. Structured knowledge distillation for semantic segmentation[C]//Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition. 2019: 2604-2613.
\bibitem{ref28}
Zhu J, Tang S, Chen D, et al. Complementary relation contrastive distillation[C]//Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition. 2021: 9260-9269.
\bibitem{ref29}
Tian Y, Krishnan D, Isola P. Contrastive multiview coding[C]//European conference on computer vision. Springer, Cham, 2020: 776-794.
\bibitem{ref30}
Tian Y, Krishnan D, Isola P. Contrastive representation distillation[J]. arXiv preprint arXiv:1910.10699, 2019.
\bibitem{ref31}
Chen Y, Xian Y, Koepke A, et al. Distilling audio-visual knowledge by compositional contrastive learning[C]//Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition. 2021: 7016-7025.
\bibitem{ref32}
Berry R B, Brooks R, Gamaldo C E, et al. The AASM manual for the scoring of sleep and associated events[J]. Rules, Terminology and Technical Specifications, Darien, Illinois, American Academy of Sleep Medicine, 2012, 176: 2012.
\bibitem{ref33}
Jia Z, Lin Y, Wang J, et al. SalientSleepNet: Multimodal salient wave detection network for sleep staging[J]. arXiv preprint arXiv:2105.13864, 2021.
\bibitem{ref34}
Soomro K, Zamir A R, Shah M. A dataset of 101 human action classes from videos in the wild[J]. Center for Research in Computer Vision, 2012, 2(11).
\bibitem{ref35}
Velickovic P, Cucurull G, Casanova A, et al. Graph attention networks[J]. stat, 2017, 1050: 20.
\bibitem{ref36}
Wang S, Yu L, Li C, et al. Learning from extrinsic and intrinsic supervisions for domain generalization[C]//European Conference on Computer Vision. Springer, Cham, 2020: 159-176.
\bibitem{ref37}
Tran D, Wang H, Torresani L, et al. A closer look at spatiotemporal convolutions for action recognition[C]//Proceedings of the IEEE conference on Computer Vision and Pattern Recognition. 2018: 6450-6459.
\bibitem{ref38}
Hara K, Kataoka H, Satoh Y. Learning spatio-temporal features with 3d residual networks for action recognition[C]//Proceedings of the IEEE international conference on computer vision workshops. 2017: 3154-3160.
\bibitem{ref39}
Carreira J, Noland E, Hillier C, et al. A short note on the kinetics-700 human action dataset[J]. arXiv preprint arXiv:1907.06987, 2019.
\bibitem{ref40}
Monfort M, Andonian A, Zhou B, et al. Moments in time dataset: one million videos for event understanding[J]. IEEE transactions on pattern analysis and machine intelligence, 2019, 42(2): 502-508.
\bibitem{ref41}
Cohen J. A coefficient of agreement for nominal scales[J]. Educational and psychological measurement, 1960, 20(1): 37-46.
\bibitem{ref42}
Romero A, Ballas N, Kahou S E, et al. Fitnets: Hints for thin deep nets[J]. arXiv preprint arXiv:1412.6550, 2014.
\bibitem{ref43}
Passalis N, Tefas A. Learning deep representations with probabilistic knowledge transfer[C]//Proceedings of the European Conference on Computer Vision (ECCV). 2018: 268-284.
\bibitem{ref44}
Passalis N, Tzelepi M, Tefas A. Heterogeneous knowledge distillation using information flow modeling[C]//Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition. 2020: 2339-2348.
\bibitem{ref45}
Tian Y, Krishnan D, Isola P. Contrastive multiview coding[C]//European conference on computer vision. Springer, Cham, 2020: 776-794.

\bibitem{ref46}
Supratak A, Dong H, Wu C, et al. DeepSleepNet: A model for automatic sleep stage scoring based on raw single-channel EEG[J]. IEEE Transactions on Neural Systems and Rehabilitation Engineering, 2017, 25(11): 1998-2008.
\bibitem{ref47}
Jia Z, Cai X, Jiao Z. Multi-modal physiological signals based squeeze-and-excitation network with domain adversarial learning for sleep staging[J]. IEEE Sensors Journal, 2022, 22(4): 3464-3471.
\bibitem{ref48}
Kong Q, Cao Y, Iqbal T, et al. Panns: Large-scale pretrained audio neural networks for audio pattern recognition[J]. IEEE/ACM Transactions on Audio, Speech, and Language Processing, 2020, 28: 2880-2894.
\bibitem{ref49}
Gemmeke J F, Ellis D P W, Freedman D, et al. Audio set: An ontology and human-labeled dataset for audio events[C]//2017 IEEE international conference on acoustics, speech and signal processing (ICASSP). IEEE, 2017: 776-780.
\bibitem{ref50}
Chen X, He J, Wu X, et al. Sleep staging by bidirectional long short-term memory convolution neural network[J]. Future Generation Computer Systems, 2020, 109: 188-196.
\bibitem{ref51}
Van der Maaten L, Hinton G. Visualizing data using t-SNE[J]. Journal of machine learning research, 2008, 9(11).

==> samples/tables/NEW_ab.tex <==
\begin{table}[]
 \small
 \centering
\caption{The complete ablation on loss formulation. Metric:Top1 accuracy (\%).}
\setlength\tabcolsep{0.55pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{cl|lcl|lcl|lcllcllcllcllc}
\hline
\multicolumn{1}{l}{} &  &  & \multicolumn{1}{l}{}        &  &  & \multicolumn{1}{l}{} &  & \multicolumn{14}{c}{Per-class Accuracy}                                                                                                                                                      \\
Methods              &  &  & Module                      &  &  & Accuracy             &  &  & W             &                       &  & N1            &                       &  & N2            &                       &  & N3            &                       &  & REM           \\ \hline
baseline             &  &  & L_{CE}                      &  &  & 52.2                 &  &  & 64.7          & \multicolumn{1}{l|}{} &  & 40.3          & \multicolumn{1}{l|}{} &  & 48.4          & \multicolumn{1}{l|}{} &  & 47.8          & \multicolumn{1}{l|}{} &  & 57.3          \\
v1                   &  &  & L_{CE}+L_{C}+L_{JSD}        &  &  & 56.1                 &  &  & 68.7          & \multicolumn{1}{l|}{} &  & 43.8          & \multicolumn{1}{l|}{} &  & 52.0          & \multicolumn{1}{l|}{} &  & 51.4          & \multicolumn{1}{l|}{} &  & 61.2          \\
v2                   &  &  & L_{CE}+L_{D}+L_{C}          &  &  & 62.3                 &  &  & 73.4          & \multicolumn{1}{l|}{} &  & 49.0          & \multicolumn{1}{l|}{} &  & 58.0          & \multicolumn{1}{l|}{} &  & 57.2          & \multicolumn{1}{l|}{} &  & 65.8          \\
v3                   &  &  & L_{CE}+L_{D}+L_{JSD}        &  &  & 60.1                 &  &  & 71.5          & \multicolumn{1}{l|}{} &  & 45.6          & \multicolumn{1}{l|}{} &  & 55.4          & \multicolumn{1}{l|}{} &  & 54.5          & \multicolumn{1}{l|}{} &  & 63.6          \\
v4                   &  &  & L_{CE}+L_{D}+L_{JSD}+L_{C'} &  &  & 61.1                 &  &  & 72.4          & \multicolumn{1}{l|}{} &  & 46.8          & \multicolumn{1}{l|}{} &  & 56.7          & \multicolumn{1}{l|}{} &  & 55.8          & \multicolumn{1}{l|}{} &  & 64.6          \\
Ours                 &  &  & L_{CE}+L_{D}+L_{C}+L_{JSD}  &  &  & \textbf{64.4}        &  &  & \textbf{75.6} & \multicolumn{1}{l|}{} &  & \textbf{51.0} & \multicolumn{1}{l|}{} &  & \textbf{60.2} & \multicolumn{1}{l|}{} &  & \textbf{59.3} & \multicolumn{1}{l|}{} &  & \textbf{67.8} \\ \hline
    \end{tabular}}
\label{tab: newab}
\end{table}

==> samples/tables/mainresults.tex <==
\begin{table*}[t]
\small
\caption{Comparison Results (\%) among SACD and State-of-art Models. The Best Values on $S^3VE$ Dataset Are Highlighted in Bold.}
\centering
{
\begin{tabular}{cl|lclllll|lllllllllll}
\hline
\multicolumn{2}{l|}{} & \multicolumn{7}{c|}{Overall Metrics}                                                       & \multicolumn{11}{c}{Per-class Accuracy}                                                                                            \\
Methods           &   &  & \multicolumn{1}{l}{Accuracy} &  & \multicolumn{1}{c}{MF1} &  & \multicolumn{1}{c}{$\kappa$} &  &  & \multicolumn{1}{c}{W} &  & \multicolumn{1}{c}{N1} &  & \multicolumn{1}{c}{N2} &  & \multicolumn{1}{c}{N3} &  & REM           &  \\ \hline
Baseline R(2+1)D  &   &  & 52.5                         &  & 46.6                    &  & 0.47                  &  &  & 64.7                  &  & 41.3                   &  & 48.4                   &  & 47.8                   &  & 57.3          &  \\
Baseline R3D      &   &  & 52.8                         &  & 46.9                    &  & 0.37                  &  &  & 64.7                  &  & 41.4                   &  & 49.0                   &  & 48.0                   &  & 58.0          &  \\
Fitnet            &   &  & 56.1                         &  & 49.9                    &  & 0.49                  &  &  & 68.5                  &  & 47.2                   &  & 55.9                   &  & 53.8                   &  & 61.8          &  \\
PKT               &   &  & 58.1                         &  & 51.2                    &  & 0.53                  &  &  & 71.2                  &  & 47.8                   &  & 56.3                   &  & 54.0                   &  & 62.9          &  \\
CRD               &   &  & 62.3                         &  & 55.8                    &  & 0.56                  &  &  & 73.8                  &  & 49.8                   &  & 58.8                   &  & 57.1                   &  & 66.4          &  \\
IFD               &   &  & 61.1                         &  & 54.0                    &  & 0.57                  &  &  & 73.0                  &  & 49.9                   &  & 58.8                   &  & 57.1                   &  & 65.1          &  \\
CMC               &   &  & 58.9                         &  & 53.1                    &  & 0.53                  &  &  & 71.5                  &  & 46.2                   &  & 56.9                   &  & 55.0                   &  & 63.2          &  \\
CCL               &   &  & 62.3                         &  & 57.0                    &  & 0.56                  &  &  & 74.4                  &  & 50,1                   &  & 58.7                   &  & 53.8                   &  & 64.7          &  \\
SACD(ours)        &   &  & \textbf{64.4}                &  & \textbf{58.9}           &  & \textbf{0.60}         &  &  & \textbf{75.6}         &  & \textbf{51.0}          &  & \textbf{60.2}          &  & \textbf{59.3}          &  & \textbf{67.8} &  \\ \hline
\end{tabular}
}
\label{tab:maintab}
\end{table*}

==> samples/tables/tab_analysisab.tex <==
\begin{table}[]

 \small
 \centering
\caption{The complete ablation on loss formulation. Metric:Top1 accuracy (\%).}
\setlength\tabcolsep{0.55pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
Methods          & \begin{tabular}[c]{@{}c@{}}Five-class\\ (W/N1/N2/N3/REM)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Three-class\\ (W/N/REM)\end{tabular} & W    & N1   & N2            & N3   & REM  \\ \hline
Baseline R(2+1)D & 52.2                                                                 & 76.1                                                           & 64.7 & 45.3 & 48.4          & 47.8 & 57.3 \\ \hline
SACD w $L_D$        & 56.1                                                                 & 79.2                                                           & 68.7 & 48.8 & 52.0          & 51.4 & 61.2 \\ \hline
SACD w/o $L_C'$     & 61.1                                                                 & 82.4                                                           & 72.4 & 52.8 & 56.7          & 55.8 & 64.6 \\ \hline
SACD w/o $L_C$      & 60.1                                                                 & 81.6                                                           & 71.5 & 51.6 & 55.4          & 54.5 & 63.6 \\ \hline
SACD w/o $L_{JSD}$    & 62.3                                                                 & 83.9                                                           & 73.4 & 55.0 & 58.0          & 57.2 & 65.8 \\ \hline
SACD             & 64.4                                                                 & 86.1                                                           & 75.6 & 57.0 & 60.2          & 59.3 & 67.8 \\ \hline
\end{tabular}
}
\label{tab:supal}
\end{table}

==> samples/tables/tab_sup4.tex <==
\begin{table}[]


 \small
 \centering
\caption{Sleep stage classification for IR+EEG. Metric:Top1 accuracy (\%).
   \textit{ (In Experiment A, We use a single fully connected layer as the prediction head;  in Experiment B, We use three fully connected layer as the prediction head.)}}
\setlength\tabcolsep{0.55pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c}
\hline
Methods      & \begin{tabular}[c]{@{}c@{}}Fiveclass\\ (W/N1/N2/N3/REM)\end{tabular} & Stage W & Stage N1 & Stage N2 & Stage N3       & Stage REM \\ \hline
Baseline R3D & 52.8                                                                 & 64.7    & 45.3     & 48.4     & 47.8           & 57.3      \\ \hline
Baseline EEG & 78.8                                                                 & 92.83   & 54.18    & 74.16    & 78.74          & 70.48     \\ \hline
Experiment A & 79.3                                                                 & 92.99   & 54.80    & 74.50    & \textit{78.72} & 70.83     \\ \hline
Experiment B & 80.1                                                                 & 93.90   & 55.50    & 75.31    & 79.80          & 71.82     \\ \hline
\end{tabular}}
\label{tab:ir+eeg}
\end{table}

==> samples/tables/tab_sup5.tex <==
\begin{table}[]



 \small
 \centering
\caption{Evaluation of different hyperparameters. Metric:Top1 accuracy (\%).}
\setlength\tabcolsep{0.55pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|c|c|c}
\hline
$\lambda_1$:$\lambda_2$:$\lambda_3$& 0.1:0.1:0.1 & 0.1:0.5:0.5    & 0.5:0.1:0.5 & 0.5:0.5:0.1 \\ \hline
Results         & 59.8        & 62.4           & 60.8        & 61.9        \\ \hline
$\lambda_1$:$\lambda_2$:$\lambda_3$ & 0.5:0.5:0.5 & 0.5:0.5:1      & 0.5:1:0.5   & 0.5:1:1     \\ \hline
Results         & 63.0        & 63.3           & 63.8        & 64.40       \\ \hline
$\lambda_1$:$\lambda_2$:$\lambda_3$ & 1:0.5:1     & 1:1:0.5        & 1:1:1       & 10:10:10    \\ \hline
Results         & 63.2        & 63.7           & 64.2        & 59.3        \\ \hline
$\lambda_1$:$\lambda_2$:$\lambda_3$ & 0.8:1:1     & 0.75:1:1       & 0.6:1:1     & 0.65:1:1     \\ \hline
Results         & 64.42       & \textbf{64.55} & 64.43       & 64.48       \\ \hline
\end{tabular}}
\label{tab:hyperp}
\end{table}

==> samples/tables/table_2.tex <==
\begin{table}[]
 \small
 \centering
\caption{Video classification on $S^3VE$. Metric:Top1 accuracy (\%).}
\setlength\tabcolsep{0.55pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccccllll}
\cline{1-8}
\multicolumn{1}{l|}{Methods}          & \begin{tabular}[c]{@{}c@{}}5-CLASS\\ (W/N1/N2/N3/REM)\end{tabular} & \begin{tabular}[c]{@{}c@{}}3-CLASS\\ (W/N/REM)\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}CLASS\\  W\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}CLASS\\  N1\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}CLASS\\ N2\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}CLASS\\ N3\end{tabular}} & \begin{tabular}[c]{@{}c@{}}CLASS\\ R\end{tabular} &  &  &  &  \\ \cline{1-8}
\multicolumn{1}{l|}{Baseline-R(2+1)D} & 52.5                                                               & 76.1                                                        & \multicolumn{1}{c|}{64.7}                                               & \multicolumn{1}{c|}{45.3}                                                & \multicolumn{1}{c|}{48.4}                                               & \multicolumn{1}{c|}{47.8}                                               & 57.3                                              &  &  &  &  \\
\multicolumn{1}{l|}{Baseline-R3D}     & 52.8                                                               & 76.7                                                        & \multicolumn{1}{c|}{64.7}                                               & \multicolumn{1}{c|}{45.4}                                                & \multicolumn{1}{c|}{49.0}                                               & \multicolumn{1}{c|}{48.0}                                               & 58.0                                              &  &  &  &  \\
\multicolumn{1}{l|}{Fitnet}           & 56.1                                                               & 80.8                                                        & \multicolumn{1}{c|}{68.5}                                               & \multicolumn{1}{c|}{51.2}                                                & \multicolumn{1}{c|}{55.9}                                               & \multicolumn{1}{c|}{53.8}                                               & 61.8                                              &  &  &  &  \\
\multicolumn{1}{l|}{PKT}              & 58.1                                                               & 82.6                                                        & \multicolumn{1}{c|}{71.2}                                               & \multicolumn{1}{c|}{51.8}                                                & \multicolumn{1}{c|}{56.3}                                               & \multicolumn{1}{c|}{54.0}                                               & 62.9                                              &  &  &  &  \\
\multicolumn{1}{l|}{CRD}              & \textit{62.3}                                                      & 84.1                                                        & \multicolumn{1}{c|}{74.2}                                               & \multicolumn{1}{c|}{55.8}                                                & \multicolumn{1}{c|}{58.8}                                               & \multicolumn{1}{c|}{57.1}                                               & 66.4                                              &  &  &  &  \\
\multicolumn{1}{l|}{IFD}              & 61.1                                                               & 83.2                                                        & \multicolumn{1}{c|}{73.0}                                               & \multicolumn{1}{c|}{53.9}                                                & \multicolumn{1}{c|}{58.8}                                               & \multicolumn{1}{c|}{57.1}                                               & 65.1                                              &  &  &  &  \\
\multicolumn{1}{l|}{CMC}              & 58.9                                                               & 82.8                                                        & \multicolumn{1}{c|}{71.5}                                               & \multicolumn{1}{c|}{52.2}                                                & \multicolumn{1}{c|}{56.9}                                               & \multicolumn{1}{c|}{55.0}                                               & 63.2                                              &  &  &  &  \\
\multicolumn{1}{l|}{CCL}              & \textit{62.3}                                                      & 84.6                                                        & \multicolumn{1}{c|}{74.4}                                               & \multicolumn{1}{c|}{56.1}                                                & \multicolumn{1}{c|}{58.7}                                               & \multicolumn{1}{c|}{57.8}                                               & 66.7                                              &  &  &  &  \\
\multicolumn{1}{l|}{Ours(SACD)}       & \textbf{64.4}                                                      & \textbf{86.1}                                               & \multicolumn{1}{c|}{\textbf{75.6}}                                      & \multicolumn{1}{c|}{\textbf{57.0}}                                       & \multicolumn{1}{c|}{\textbf{60.2}}                                      & \multicolumn{1}{c|}{\textbf{59.3}}                                      & \textbf{67.8}                                     &  &  &  &  \\ \cline{1-8}
                                      & \multicolumn{1}{l}{}                                               & \multicolumn{1}{l}{}                                        & \multicolumn{1}{l}{}                                                    & \multicolumn{1}{l}{}                                                     & \multicolumn{1}{l}{}                                                    & \multicolumn{1}{l}{}                                                    & \multicolumn{1}{l}{}                              &  &  &  &  \\
                                      & \multicolumn{1}{l}{}                                               & \multicolumn{1}{l}{}                                        & \multicolumn{1}{l}{}                                                    & \multicolumn{1}{l}{}                                                     & \multicolumn{1}{l}{}                                                    & \multicolumn{1}{l}{}                                                    & \multicolumn{1}{l}{}                              &  &  &  & 
\end{tabular}}
\label{tab:allresults}
\end{table}


==> samples/tables/table_3.tex <==
\begin{table}[]
\small

 \centering
\caption{Video classification on UCF51. Metric:Top1 accuracy (\%).}

\resizebox{\linewidth}{!}{
\begin{tabular}{c|ccccccccc}
\cline{1-9}
Methods & Baseline-(2+1)D & Fitnet & PKT  & RKD  & CRD  & CMC  & CCL           & Ours(SACD)    &  \\ \cline{1-9}
UCF51   & 57.5            & 48.4   & 53.2 & 53.0 & 60.3 & 59.2 & \textit{64.9} & \textbf{66.0} &  \\ \cline{1-9}
\end{tabular}
}
\label{tab:allresults123}
\end{table}

